Connecting indefinite causal order processes to composable quantum protocols in a spacetime

Process matrices are a framework to model causal relations in the absence of a well-defined acyclic causal order. The framework is very general and does not even assume the existence of a background spacetime. As a result, it is an open question how the framework should be interpreted physically and how and even if composition can be defined. On the other hand, so-called causal boxes define a framework that allows for arbitrary composition. In this work, we treat quantum circuits with quantum control of causal order (QC-QC), a subset of process matrices, which can be interpreted as generalized quantum circuits, and process box, a subset of causal boxes, which can be interpreted as processes. We analyze their state spaces and define a notion of operational equivalence between QC-QCs and process boxes based on this analysis. We then explicitly construct for each QC-QC an operationally equivalent process box. This allows us to define composition of QC-QCs in terms of composition of causal boxes which is well-defined. We further show that process boxes admit a unitary extension and conjecture that the background spacetime can be assumed to have a specific simple form. Based on this conjecture, we construct an operationally equivalent QC-QC for each process box. Our results indicate that the only class of processes that can be physically implemented in a fixed background spacetime are those that can be interpreted as quantum circuits with quantum controlled superpositions of orders. Further, they also reveal that the composability issue can be resolved by embedding processes in a spacetime structure. This in turn sheds light on the connection between physical realizability in a spacetime and composability.

==> macros.tex <==

% This package provides several macros for Quantum Information Theory, example boxes, prettifying in general 

% Adapted from Marco Tomamichel's 2011 macros by Lidia del Rio 2014, Christopher Portmann, Nuriya Nurgalieva, V. Vilasini (2017-2021).


% language input
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[T1]{fontenc}
\usepackage{afterpage}
%\usepackage{ntheorem}
\usepackage{natbib}

\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{graphicx}
\usepackage[ colorlinks = true, 
             linkcolor = MidnightBlue,
             urlcolor  = MidnightBlue,
             citecolor = orange,
             anchorcolor = ForestGreen,
]{hyperref} 
\usepackage{float}

\makeatletter
\def\mathcolor#1#{\@mathcolor{#1}}
\def\@mathcolor#1#2#3{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}
\makeatother

% additional fonts
\usepackage[sans]{dsfont} % contains font for identity character
\usepackage{bbm}
\usepackage[mathscr]{euscript}
\usepackage{cancel} %to strike out things
\usepackage{amsfonts}


%boxes and theorems
\usepackage{tcolorbox}
\tcbuselibrary{theorems} 

% more stuff
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{units}
\usepackage{framed}
\usepackage{mdframed}
\usepackage{thmtools, thm-restate} %pretty  and restatable theorems
\usepackage{ucs}
\usepackage{subcaption}
\usepackage{fullpage}
\usepackage{csquotes}
\usepackage{epigraph}


%break into cloumns
\usepackage{multicol}
\setlength{\columnsep}{0.5cm}

%enumerate in line
\usepackage{enumerate}
%\usepackage[inline]{enumitem}

% modified by Vilasini
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  tikz arrows, commutative diagrams, decorations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%tikz
\usepackage{tikz}
\usetikzlibrary{arrows}
\usepackage{rotating, xcolor}
\usetikzlibrary{shapes}
\usetikzlibrary{hobby}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{calc,intersections,through,backgrounds}
\usetikzlibrary{decorations.pathreplacing,angles,quotes}
\usetikzlibrary{arrows,decorations.markings}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{snakes} 
\usepackage{tikz-cd}
\tikzset{degil/.style={
            decoration={markings,
            mark= at position 0.5 with {
                  \node[transform shape] (tempnode) {$\setminus$};
                  %\draw[thick] (tempnode.north east) -- (tempnode.south west);
                  }
              },
              postaction={decorate}
}
}


%caption
\captionsetup[subfigure]{skip=5pt}
\captionsetup[figure]{skip=10pt}
\captionsetup[subfigure]{justification=centering}



% .......................... boxes ...........


%default colours
\tcbset{colback=orange!5,colframe=orange!75!yellow, 
%colbacktitle=orange!65!white, 
fonttitle= \bfseries, float=htb}



%..................................................

% Colours
	\newcommand{\red}[1]{\textcolor{Red}{#1}}
	\newcommand{\blue}[1]{\textcolor{Blue}{#1}}
	\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
	\newcommand{\pink}[1]{\textcolor{Magenta}{#1}}
	\newcommand{\yellow}[1]{\textcolor{Yellow}{#1}}
	\newcommand{\orange}[1]{\textcolor{Orange}{#1}}
	
 

\DeclareMathOperator{\tr}{tr}
\newcommand{\C}{\mathcal}



%comments
\newcommand{\ms}[1]{\textcolor{black!60!green}{ [#1]}}
\newcommand{\vv}[1]{\textcolor{blue}{ [#1]}}
	
% Referencing equations and figures
	\newcommand{\eref}[1]{Eq.\ \ref{#1}}
	\newcommand{\fref}[1]{Fig.\ \ref{#1}}
	
	
% ........................................................
	
	
% ........... Hilbert spaces and states  ...............
	
% Dirac notation
    \newcommand{\ket}[1]{\vert  #1 \rangle}
    \newcommand{\bra}[1]{\langle #1 |}
    \newcommand{\inprod}[2]{\langle #1 | #2 \rangle}
	\newcommand{\proj}[2]{\ket{#1}\bra{#2}}
	\newcommand{\pure}[1]{\proj{#1}{#1}}
 

% Hilbert spaces
	\newcommand{\hilbert}{\mathcal{H}}
	\newcommand{\composed}{\mathcal{H}_A  \otimes \mathcal{H}_R}
	


% ..... operators and maps .....  

% Powerset
	\newcommand{\Powerset}[1]{\operatorname{Powerset}(#1)} 

% Span
	\newcommand{\Span}[1]{\operatorname{Span}(#1)} 
	
% Diagonal 
\newcommand*{\diag}{\operatorname{diag}}


%Identity operator
	\newcommand{\id}{\mathbbm{1}}
    %\newcommand{\id}{id}

% % Trace
	\newcommand{\tr}{\operatorname{Tr}  }
	\DeclareMathOperator{\Tr}{Tr}

%TPCPMs
\newcommand*{\I}{\mathcal{I}}
\newcommand*{\E}{\mathcal{E}}
\newcommand*{\cM}{\mathcal{M}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\OO}[1]{\mathcal{O} \left( #1 \right) }
% % \newcommand{\ham}{\mathcal{H}}




% ...........  general maths  .................

% % Vectors
	\renewcommand{\vec}[1]{\mathbf{#1}}
	\newcommand{\vecop}[1]{\hat{\mathbf{#1}}}


%Set
	\newcommand{\set}[1]{\left\{ #1 \right\}}


% % Absolute value
	\newcommand{\abs}[1]{\left| #1 \right|}

% Matrices
	\newcommand{\matrixTwo}[1]{
		\left( 
			\begin{array}{c c}
				#1
			\end{array}
		\right)
		}
	\newcommand{\matrixN}[2]{
		\left( 
			\begin{array}{#1}
				#2
			\end{array}
		\right)
		}

% Probability
	%\newcommand{\prob}{\mathcal{P}}
	%\newcommand{\Prob}[1]{\mbox{Prob} \left[ #1 \right]}
	% Long probabilities
	\newcommand{\prob}[2]{
		\Pr_{#1}
		\left\{
			\begin{array}{l}
				#2
			\end{array}
		\right\}
		}

% ............................................

% Little things
	\newcommand{\ie}{i.e., }
	\newcommand{\etal}{et al.\ }
	\newcommand{\cj}{Choi-Jamio\l{}kowski }
	%\newcommand{\iid}{i.i.d.\  }

	\newcommand*{\eps}{\varepsilon}
	\newcommand*{\half}{\frac{1}{2}}
    \newcommand{\Ss}{state-space }
    \newcommand{\constr}[1]{\overset{#1}{\to}}




% added by Christopher
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  multiple links to the same footnote
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\footnoteremember}[2]{\footnote{\label{#1}#2}\newcounter{#1}\setcounter{#1}{\value{footnote}}}
\newcommand{\footnoterecall}[1]{\hyperref[#1]{\footnotemark[\value{#1}]}}



% added by Nuriya, Vilasini
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  clever ref, proof
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[capitalise, noabbrev]{cleveref}
\newenvironment{proof}{\paragraph{Proof:}}{\hfill$\square$}

%\input{Qcircuit}
\usepackage[page]{totalcount}
%\usepackage{thmtools, thm-restate}

\usetikzlibrary{shapes}
\usetikzlibrary{hobby}
\usetikzlibrary{decorations.markings}

% added by Vilasini
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  theorem environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
%\declaretheorem[style=boxed]{definition}



\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1\langle}\)}%
  \mathopen{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1\rangle}\)}%
  \mathclose{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\makeatother


